A mixed finite-element, finite-volume, semi-implicit discretisation for atmospheric dynamics: Spherical geometry

The reformulation of the Met Office's dynamical core for weather and climate prediction previously described by the authors is extended to spherical domains using a cubed-sphere mesh. This paper updates the semi-implicit mixed finite-element formulation to be suitable for spherical domains. In particular the finite-volume transport scheme is extended to take account of non-uniform, non-orthogonal meshes and uses an advective-then-flux formulation so that increment from the transport scheme is linear in the divergence. The resulting model is then applied to a standard set of dry dynamical core tests and compared to the existing semi-implicit semi-Lagrangian dynamical core currently used in the Met Office's operational model.

==> figures/local_coordinates.tex <==

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.75]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Curve Lines [id:da4574882998019949] 
\draw    (131,51) .. controls (190,43) and (270,57) .. (377,126) ;
%Curve Lines [id:da5908904733453539] 
\draw    (123,101) .. controls (182,93) and (262,107) .. (369,176) ;
%Curve Lines [id:da5065591404417982] 
\draw    (108,156) .. controls (167,148) and (247,162) .. (354,231) ;
%Curve Lines [id:da9209310648063838] 
\draw    (99,210) .. controls (158,202) and (238,216) .. (345,285) ;
%Curve Lines [id:da6269502645843523] 
\draw    (155,20) .. controls (181,52) and (158,173) .. (118,266) ;
%Curve Lines [id:da4907376821808376] 
\draw    (219,28) .. controls (245,60) and (222,181) .. (182,274) ;
%Curve Lines [id:da7155932551862823] 
\draw    (282,38) .. controls (308,70) and (285,191) .. (245,284) ;
%Curve Lines [id:da05661336015729068] 
\draw    (334,63) .. controls (360,95) and (337,216) .. (297,309) ;
%Shape: Axis 2D [id:dp7101472983711647] 
\draw  (31,287) -- (131,287)(41,197) -- (41,297) (124,282) -- (131,287) -- (124,292) (36,204) -- (41,197) -- (46,204)  ;
%Straight Lines [id:da657831629713387] 
\draw    (41,287) -- (99.34,248.11) ;
\draw [shift={(101,247)}, rotate = 146.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Axis 2D [id:dp5187940266481246] 
\draw  (242.47,146.67) -- (314.04,172.67)(270.84,91.68) -- (248.34,153.61) (309.17,165.58) -- (314.04,172.67) -- (305.76,174.98) (263.75,96.56) -- (270.84,91.68) -- (273.15,99.97)  ;
%Shape: Circle [id:dp16521074111945366] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (243.38,149.36) .. controls (243.38,145.77) and (246.29,142.86) .. (249.88,142.86) .. controls (253.47,142.86) and (256.38,145.77) .. (256.38,149.36) .. controls (256.38,152.95) and (253.47,155.86) .. (249.88,155.86) .. controls (246.29,155.86) and (243.38,152.95) .. (243.38,149.36) -- cycle ;
%Shape: Circle [id:dp03457970326570603] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (303.88,102.36) .. controls (303.88,98.77) and (306.79,95.86) .. (310.38,95.86) .. controls (313.97,95.86) and (316.88,98.77) .. (316.88,102.36) .. controls (316.88,105.95) and (313.97,108.86) .. (310.38,108.86) .. controls (306.79,108.86) and (303.88,105.95) .. (303.88,102.36) -- cycle ;
%Straight Lines [id:da5383490301171021] 
\draw    (310.38,102.36) -- (249.88,149.36) ;

% Text Node
\draw (317,164.4) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (274,76.4) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (319.88,105.76) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{x}_{i}$};
% Text Node
\draw (251.88,159.26) node [anchor=north west][inner sep=0.75pt]    {$\mathbf{x}_{0}$};
% Text Node
\draw (273,128.4) node [anchor=north west][inner sep=0.75pt]    {$s$};
% Text Node
\draw (134,278.4) node [anchor=north west][inner sep=0.75pt]    {$X$};
% Text Node
\draw (104,235.4) node [anchor=north west][inner sep=0.75pt]    {$Y$};
% Text Node
\draw (36,174.4) node [anchor=north west][inner sep=0.75pt]    {$Z$};


\end{tikzpicture}
